Interpolatory-based data-driven pulsed fluidic actuator control design and experimental validation

Pulsed fluidic actuators play a central role in the fluid flow experimental control strategy to achieve better performances of aeronautic devices. In this paper, we demonstrate, through an experimental test bench, how the interpolatory-based Loewner Data-Driven Control (L-DDC) framework is an appropriate tool for accurately controlling the outflow velocity of this family of actuators. L-DDC combines the concept of ideal controller with the Loewner framework in a single data-driven rationale, appropriate to experimental users. The contributions of the paper are, first, to emphasise the simplicity and versatility of such a data-driven rationale in a constrained experimental setup, and second, to solve some practical fluid engineers concerns by detailing the complete workflow and key ingredients for successfully implementing a pulsed fluidic actuator controller from the data acquisition to the control implementation and validation stages.

==> sec_intro.tex <==
%\subsection{Fluidic actuator control: context and motivations}

The design of active closed-loop flow controllers constitutes an important field of research in fluid mechanics. % using an adequate sensor-actuator couple relation. 
Active flow control is considered in many applications among which flows over open cavities (see \eg \cite{LeclercqJFM:2019}) and backward facing steps, boundary layer flows (see \eg \cite{Sipp:2016}), flows over airfoils or again combustion processes with varying objectives: maintain laminarity or delay transition to turbulence, decrease turbulence level, reduce noise, increase lift and decrease drag, enhance mixing and heat release \etc
%As an illustration, reader may refer to \cite{LeclercqJFM:2019} where flow control over a oscillatory configuration is considered, or \cite{Sipp:2016}, where flow control over an amplifier case is addressed. 
Without detailing the specificity and the control methodology employed in each cases, in most of these contributions and the references therein, both the sensor(s) and the actuator(s) are supposed to be lumped and ideal. By this, one intends that the sensors are capable to deliver instantaneous and accurate measurements, while the actuators are able to deliver the exact control signals computed by the flow controller (\eg with no delay, no noise, continuous control signal and unbounded intervals, \etc). These developments are relevant for academic and methodological purposes. However, in order to move towards experimental applications and expect real-life validations, it is essential to consider a realistic setup instead of these idealized versions. Therefore, accurate consideration of the actuator-sensor combination is absolutely necessary. This constitutes the core of this paper.% (see also \cite{}). % one is interested in  accurately considering the actuators and sensors couples

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./OL_inoutAvg.pdf}
    \caption{Extract of the open-loop data collected on the experimental setup. The output response ${\y}(t_{k/N})$ (solid orange) is obtained by feeding the \textbf{PFA} with an on/off PRBS input signal ${\u}(t_{k/N})$ (dotted blue). The averaged output $\overline{\y}(t_{k})$ (solid black) results in averaging ${\y}(t_{k/N})$ over $N$ samples. The actuator needs to be controlled to fit the reference sent by the outer-loop controller and deliver an almost continuous mean value.}
    \label{fig:OLinout}
\end{figure}

\begin{figure}[h!]
    \centering
    \scalebox{.5}{
    %%%%%%%%%%%%%%\input{figures/controlLoopMixed}
    \tikzstyle{block} = [draw, thick,fill=bleuONERA!20, rectangle, minimum height=3em, minimum width=6em,rounded corners]
\tikzstyle{block2} = [thick,rectangle, minimum height=3em, minimum width=6em,rounded corners]
\tikzstyle{sum} = [draw, thick,fill=bleuONERA!20, circle, node distance=1cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thick,black}]
\tikzstyle{connector} = [->,thick]
% The block diagram code is probably more verbose than necessary
\begin{tikzpicture}[auto, node distance=2cm,>=latex']
    % We start by placing the blocks
    \node [input, name=input] {};
    \node [sum, right of=input] (sum) {};
    \node [block, right of=sum, node distance=3cm] (controller) {\textbf{Controller} $\mathbf K(z)$};
    \node [pinstyle, above of=controller, node distance=1.2cm] (samplingK) {$f_{s2}$};
    \draw [connector] (samplingK) -- node[name=hK] {} (controller.90);
    \node [block, right of=controller, node distance=4cm] (pwm) {\textbf{PWM}};
    \node [pinstyle, above of=pwm, node distance=1.2cm] (samplingPWM) {$f_{s1}=N f_{s2}$};
    \draw [connector] (samplingPWM) -- node[name=hPW] {} (pwm.90);
    \node [block2, right of=pwm, node distance=5cm] (system) {\includegraphics[width=4cm]{./top}};%{\textbf{PFA}};
    \node [pinstyle, above of=system, node distance=2.3cm] (samplingSystem) {$f_{s1}=N f_{s2}$};
    \draw [connector] (samplingSystem) -- node[name=hPW] {} (system.90);
    \node [block, right of=system, node distance=5cm] (mean) {\textbf{Average}};
    \node [pinstyle, above of=mean, node distance=1.2cm] (samplingMean) {$f_{s2}$};
    \draw [connector] (samplingMean) -- node[name=hhPW] {} (mean.90);
    % We draw an edge between the controller and system block to 
    % calculate the coordinate u. We need it to place the measurement block. 
    \draw [connector] (controller) -- node[name=u] {${\overline \u(t_k)}$} (pwm);
    \draw [connector] (system) -- node[name=u] {$\red{\y(t_{k/N})}$} (mean);
    \node [output, right of=mean, node distance=3cm] (outputMean) {};
    % Once the nodes are placed, connecting them is easy. 
    \draw [connector] (input) -- node {$\mathbf r(t_k)$} (sum);
    \draw [connector] (sum) -- node {$\mathbf e(t_k)$} (controller);
    \draw [connector] (pwm) -- node {\red{$\mathbf u(t_{k/N})$}} (system);
    \draw [connector] (mean) -- node {$\overline \y(t_{k})$} (outputMean);
        \draw [connector] (outputMean)+(-0.3cm,0) -- ++(-0.3cm,-2cm) -| node [near start] {} (sum.south);
\end{tikzpicture}
    %%%%%%%%%%%%%%%%%%
    }
    \caption{Overview of the inner-loop considered. \textbf{Controller} $\mathbf K(z)$ is the control law to be computed (sampled at frequency $f_{s2}$), Pulsed Width Modulation (\textbf{PWM}) block transforms the continuous signal into on/off values (sampled at frequency $f_{s1}$) and \textbf{Average} block is a down-sampling  function  providing the mean value of the input signal. The system is illustrated by its top view photo, where left side represents the \textbf{PFA} and right side, the Pressure Sensor (\textbf{PS}).}
    \label{fig:closedLoopScheme}
\end{figure}

Among the different flow actuator technologies available, which may be classified as mechanical (\eg surfaces using electrical, hydraulic, morphing actuation) or fluidic (\eg pulsed or continuous blowing, synthetic jet), the pulsed fluidic actuator (\textbf{PFA}) stands as a simple, ergonomic, economic and affordable solution. The latter is therefore widely used in fluid mechanics for control application. The most widely used \textbf{PFA} type are typically valves which control the output mass flow rate / pressure issued from a reservoir at rest with fixed pressure and temperature. A considerable amount of studies can be found in the literature on the attempts, with more or less success, to control flows in various applications. While their response time and operating frequency can be high enough compared to the main characteristic time of the flow to manipulate (at least one order of magnitude larger), it is noteworthy that this class of actuators in mainly used to excite the flow within the receptivity range of its most unstable modes, namely the large-scale structures. Their level of authority is however restricted since the \textbf{PFA}, alone, acts on the flow on a limited spatial domain. In practical applications, these actuators are therefore usually installed in arrays to provide enough energy to gain authority over the considered flow region and mechanism to be controlled. Beside this, one major drawback is that they work either completely open or closed and are thus on/off systems, see Figure \ref{fig:OLinout}. To be integrated in a global flow control scheme, these actuators may be equipped with sensors measuring the current outflow velocity and be accurately controlled at high frequency with an inner controller so that the velocity of the blown air follows the reference control signal provided by the outer controller. Indeed, these actuators are not ideal as usually assumed, presenting asymmetric dynamics and noise, as shown on Figure \ref{fig:OLinout}. On the basis of the above comments, there is a need for providing practitioners and applied fluid engineers a systematic and simple approach to design a controller tailored to \textbf{PFA} devices, allowing tracking a given reference signal fed by an outer flow controller. As mentioned previously, multiple \textbf{PFA} are generally employed in parallel in practical application. Due to manufacturing and installation versatility, some discrepancies in the characteristic responses are most of the time observed between the \textbf{PFA}s installed. One additional need is therefore to also provide a methodology that can be easily applied on multiple installed devices.

The main objective of the present contribution is therefore to provide practitioners and experimental researchers a simple but yet effective methodology and practical workflow to implement pulsed fluid actuators flow controllers directly from experiments. While the contribution is more methodological rather than theoretical, authors believe that the interpolatory-based data-driven control design process presented in this paper solves practical problems faced by practitioners, namely, the complete \textbf{PFA} controller design using open-loop data collected directly on the experimental setup only (technical details can be found in \cite{KergusLCSS:2019,KergusPhD:2019}). 

The major benefit of this data-driven rationale is that the control design requires the open-loop data collected on the actuator only, allowing to account for variations and discrepancies from an actuator to an other and thus to design a control law tailored to each system. Instead of spending time and energy in an identification and control design process, the data-driven approach is less costly to deploy in practice and tailored to each actuator%\footnote{Note that in practical applications, as it it in this one, multiple \textbf{PFA} are installed in parallel. Thus, the actuator design procedure should be repeated as many time as the number of actuators and a plug-and-play method is of great interest.}
. In addition, as the proposed workflow does not require any optimisation iteration, its application remains easy in an experimental context.  Finally, except from the closed-loop objective specification, the proposed process automatically both finds the controller %$\mathbf K(z)$ 
structure and gains.%, leading to the desired closed-loop performance.


%The paper is structured as follows. 
The control and experimental setup and closed-loop architecture are described in Section \ref{sec:setup}. Section \ref{sec:method} recalls the interpolatory-driven Loewner Data-Driven Control (\textbf{L-DDC}) control design approach, and details the key steps to follow for proper implementation. Section \ref{sec:result} is devoted to the illustration and analysis of the obtained experimental results. Conclusions and comments finally close the paper in Section \ref{sec:conclusion}.



%\subsection{Contribution and paper structure}


==> sec_method.tex <==
%Given the control scheme of Figure \ref{fig:closedLoopScheme}, let us now state the main result as a controller design workflow.

\subsection{Overview of the approach and control objective}

Considering the closed-loop structure of Figure \ref{fig:closedLoopScheme}, the objective is to track a reference signal $\mathbf r(t_k)$ \textcolor{black}{up to a frequency of $f_c=5$Hz, being the maximal frequency of the outer loop (not detailed here)}. To this aim and for the simplicity and flexibility of the implementation, a frequency-domain interpolation-based data-driven approach has been chosen. The employed workflow is summed up in Algorithm \ref{workflow} and key steps are described in the remaining of this section.
\begin{algorithm}
\caption{\textbf{L-DDC} based \textbf{PFA} control design} \label{workflow}
\begin{algorithmic}[1]
\REQUIRE A desired reference closed-loop model $\mathbf{M_{f_j}}(s)$, a \textbf{PWM} frequency $f_{s1}$ and ratio $N\in\mathbb N$.
\ENSURE $\mathbf K(z)$ sampled at $f_{s2}$, leading to similar performances to $\mathbf{M_{f_j}}(s)$ when inserted in the loop.
\STATE (Section \ref{subsec:openloop}) Generate an exciting signal using a pseudo-random binary sequence denoted $\u_{\text{prbs}}(t_{k/N})$.
\STATE (Section \ref{subsec:openloop}) Excite the \textbf{PFA} system with $\u(t_{k/N})=\u_{\text{prbs}}(t_{k/N})$, collect $\y(t_{k/N})=\y_{\text{prbs}}(t_{k/N})$, and compute the mean values leading to the so-called open-loop data 
$$\{t_k,\overline \u_{\text{prbs}}(t_k),\overline{\y}_{\text{prbs}}(t_k)\}_{k=1}^M.$$
\STATE (Section \ref{subsec:openloop}) Compute the corresponding Fourier signals $\tilde\u_{\text{prbs}}(\imath\omega_i)$ and $\tilde\y_{\text{prbs}}(\imath\omega_i)$, leading to the frequency-domain experimental transfer data as 
$$
\bigg\{\imath\omega_i,\mathbf{\Phi}_i=\frac{\tilde\y_{\text{prbs}}(\imath\omega_i)}{\tilde\u_{\text{prbs}}(\imath\omega_i)}\bigg\}_{i=1}^N.
$$
\STATE (Section \ref{subsec:lddc}) Compute the ideal controller $\mathbf K^\star(\imath\omega_i)$.
\STATE (Section \ref{subsec:lddc}) Use interpolation-based data-driven model construction and obtain the full order interpolant controller $\mathbf K_{\text{full}}(s)$.
\STATE (Section \ref{subsec:lddc}) Apply rank revealing factorisation for controller order reduction leading to $\mathbf{\tilde K}(s)$.
\STATE (Section \ref{subsec:lddc}) Compute $\mathbf K(z)$, the discrete-time version $\mathbf {\tilde K}(s)$ using any discretisation method, with frequency sampling $f_{s2}=f_{s1}/N$.
\end{algorithmic}
\end{algorithm}

%\begin{remark}
%Reader should note that many data-driven control design method exist. Still it but it is not our principal objective to describe and compare them all. Interested reader can refer to \cite{Campi:2002,Formentin:2013,Formentin:2014} an references therein. Still, one major benefit of the \textbf{L-DDC} is that is does not requires controller structure $\mathbf K(z)$ to be predefined. 
%\end{remark}

\subsection{Open-loop data acquisition and frequency response construction}
\label{subsec:openloop}

The first three steps of Algorithm \ref{workflow} are now detailed and commented. These steps consists in exciting the system to obtain a relevant open-loop frequency response. %Even if the steps might appear standard, for practitioners they might be important to accurately define. 

\subsubsection{Construction of a PRBS exciting signal}

Open-loop data can be obtained using a pseudo random binary sequence signal as input of the system\footnote{Note that many other exciting signals exist but this one suits well to such a fluidic system.}. This signal consists in an on/off sequence of varying length. A "random" sequence of these signals, whose duration should last enough to reach steady state output and short enough to excite frequencies above the cut-off one of the system, is defined. The Fourier transform of the sequence $\u_{\text{prbs}}$ should be constant over the frequencies until a cut-off and is thus equivalent to a white noise over these frequencies. In practice, due to the rectangular shape of each pulse given as
\begin{equation}
    \u_{\text{prbs}}(t_{k/N}) =  \textbf{rect}_{T_{s2}}(t/T_{s2}) \left\{
    \begin{array}{ll}
    1 & \text{, $\forall t \in [-T_{s2}/2,T_{s2}/2]$} \\
    0 & \text{, elsewhere}
    \end{array}
    \right.
\end{equation}
the corresponding Fourier transform reads
\begin{equation}
    \tilde \u_{\text{prbs}}(f) = \dfrac{\sin(\pi f T_{s2})}{\pi f} = T_{s2} \mathbf{sinc}(\pi T_{s2} f),
\end{equation}
where $T_{s2}=1/f_{s2}$. Thus, harmonics can be observed every $k\pi T_{s2}$ (for $k\in \mathbb N$) and should be treated in the post-processing phase.

\subsubsection{Frequency transfer construction}

Based on the input $\u_{\text{prbs}}(t_{k/N})$ and corresponding output $\y_{\text{prbs}}(t_{k/N})$ signals, one computes the averaged signals $\overline\u_{\text{prbs}}(t_{k})$ and  $\overline\y_{\text{prbs}}(t_{k})$ and  their Fourier transform $\tilde \u_{\text{prbs}}(\imath\omega_i)$ and $\tilde \y_{\text{prbs}}(\imath\omega_i)$ respectively ($\imath=\sqrt{-1}$). Then, the cross correlation transfer of these signals are used to construct $\mathbf \Phi_i$ as 
\begin{equation}
    \mathbf \Phi_i(\imath\omega_i) = \dfrac{\tilde \y_{\text{prbs}}(\imath\omega_i)}{\tilde \u_{\text{prbs}}(\imath\omega_i)}. %= \mathbf G(\imath\omega_i)e^{\imath }
\end{equation}
In opposition to the spectral energy density, the cross (or inter-correlated) spectral density is a complex number which gain represents the interaction power and which arguments represents the phase between $\overline \u_{\text{prbs}}(t_k)$ and $\overline \y_{\text{prbs}}(t_k)$. Now the open-loop data have been collected and treated, the Loewner Data-Driven Control (\textbf{L-DDC}) process \cite{KergusLCSS:2019}, detailed in the following, can be deployed.

\subsection{Loewner Data-Driven Control}
\label{subsec:lddc}
The \textbf{L-DDC} algorithm allows to design a controller on the basis of frequency-domain data from the system to be controlled. The specifications are provided by the user as a reference model, which represents the desired closed-loop behaviour. The \textbf{L-DDC} procedure represents steps 4 to 6 of Algorithm \ref{workflow}. These three steps are detailed hereafter. %The last step 7 is simply recalled but any method can be used.

Note that, in the end, a continuous controller $\mathbf{\tilde K}(s)$ is obtained and then discretized to obtain the control law $\mathbf{K}(z)$. An hybrid version of the \textbf{L-DDC}, allowing to obtain directly a discrete controller for a continuous system, also exists and can be found in \cite{VuilleminWC:2020}, but has not been used here.

\paragraph{Reference model specification}
\label{ref_model}

As detailed in \cite{KergusLCSS:2019}, the choice of the specifications is a key aspect of the \textbf{L-DDC} procedure. Indeed, the user should take into account the performance limitations of the system to be controlled to avoid compensations of instabilities between the system and the controller, which would lead to an internally unstable closed-loop. The performance limitations of a system are determined by its own instabilities, imposing interpolatory conditions on the closed-loop to be achievable. When the system is only known through data, its instabilities, and the associated performance limitations, must be found in a data-driven way, as it is proposed in \cite{KergusLCSS:2019}, using the model-free stability analysis introduced in \cite{cooman2018model} and \cite{cooman2018estimating}.  Another option consists in using the Loewner framework as in chap. 5 of \cite{PoussotHDR:2019}: a minimal realisation is obtained through the Loewner interpolatory framework and projected onto the rational  $\mathcal{H}_\infty$ subspace of stable functions. %If the stable projection matches the minimal realisation, which is the case here as visible on Figure \ref{fig:projP}, the system is stable. The same is performed on the inverse of the available data to check if the considered system is minimum phase or not.

%\begin{figure}
    %\centering
    %\caption{Stable projection of the minimal realisation obtained from the plant's data: the PFA is stable and minimum phase.}
    %\label{fig:projP}
%\end{figure}

In the present case, the time-domain response, see Figure \ref{fig:OLinout}, allows us to conclude that the considered system is stable and minimum phase, so any stable transfer function can be used as reference model. The idea is to choose a simple model with a well-known and desirable behaviour. In the present case, a first order transfer function is chosen as
\begin{equation}
    \mathbf{M_{f_j}}(s)=\frac{1}{\frac{s}{2\pi f_j}+1},
    \label{reference_model}
\end{equation}
with $f_j\in\mathbb R_+$. The frequency $f_j$ is chosen according to the bandwidth frequency of the phenomenon to be controlled in the outer-loop. In this study, three frequencies are considered, $f_1=1$Hz, $f_3=3$Hz and $f_5=5$Hz, corresponding to reference models $\mathbf{M_{f_1}}$, $\mathbf{M_{f_3}}$ and $\mathbf{M_{f_5}}$, leading to the design of three $\mathbf K(z)$ discrete-time controllers, respectively denoted $\mathbf{K_{f_1}}(z)$, $\mathbf{K_{f_3}}(z)$ and $\mathbf{K_{f_5}}(z)$. In what follows, the design is detailed for $\mathbf{M}=\mathbf{M_{f_1}}$ only.

% les spécification en temps que 1er ordre et aussi les aspects zeros instable?

\paragraph{Ideal controller definition}

% ICI le controle idéal

Once the reference model $\mathbf{M}$ is fixed, it is possible to use the available data $\{\imath\omega_i,\mathbf{\Phi}_i\}_{i=1}^N$ to define the ideal controller $\mathbf{K}^\star$. It is the unique \lti and rational controller that would have given the desired performances during the experiment if inserted in the closed-loop. By definition, samples of its frequency response can be computed as follows, $\forall i=1\dots N$:
\begin{equation}
    \mathbf{K}^\star(\imath\omega_i) = \mathbf{\Phi}_i^{-1} \mathbf{M}(\imath\omega_i) (I - \mathbf{M}(\imath\omega_i))^{-1},
    \label{ideal_controller}
\end{equation}
where $I$ denotes the identity matrix of appropriate dimension.

Thanks to the ideal controller, the identification can be shifted from the system to the controller, and this is what makes the \textbf{L-DDC} procedure data-driven (see \eg \cite{Campi:2002}. Indeed, the main step, detailed in the next paragraph, consists in obtaining a realization $\mathbf{K}_{\text{full}}$ of the ideal controller $\mathbf{K}^\star$ that satisfies the following interpolatory conditions, $\forall i=1\dots N$:
\begin{equation}
    \mathbf{K}_{\text{full}}(\imath\omega_i) = \mathbf{K}^\star(\imath\omega_i).
    \label{CI}
\end{equation}

\paragraph{Reduced controller design}

The Loewner framework \cite{AntoulasChapSpringer:2010} allows to find a rational \lti model $\mathbf{K}_{\text{full}}$ solving problem \eqref{CI}. In addition, it is known that $\mathbf{K}_{\text{full}}$ is the smallest exact interpolating model. However, this model is often of very high order and such a controller would be too complex to be implemented. In the present case, the interpolation gives a high-order minimal realization, $n=290$, principally due to  noisy data.

Since the Loewner framework allows to control the complexity of the identified model, it is possible to obtain easily a $r$-th order reduced model $\mathbf{\tilde K}$ of the minimal realisation $\mathbf{K}_{\text{full}}$. The order of the controller becomes a tunable parameter and can be fixed by the user. The Singular Value Decomposition (\textbf{SVD}) of the Loewner pencil, on which is based the Loewner framework, allows to guess how many eigenvalues are really necessary to describe the ideal controller behaviour. In the present case, the \svd decay of the associated Loewner pencil is given on Figure \ref{fig:svdK} (see \cite{AntoulasSurvey:2016} for practical details and chap. 2 of \cite{PoussotHDR:2019} for some applications).
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./OL_sigma.pdf}
    \caption{Singular Value Decomposition of the Loewner pencil: one mode is sufficient to describe the dynamic of the ideal controller.}
    \label{fig:svdK}
\end{figure}

On Figure \ref{fig:svdK}, an order $r=3$ appears to be enough as it provides almost 80\% singular value contribution (\ie $\sigma_1+\sigma_2+\sigma_3 \approx 0.8\sum_i^n\sigma_{i=1}$). However selecting an order $r=1$ still achieves to 50\% of the information $\sigma_1 \approx 0.5\sum_i^n\sigma_{i=1}$. Such choice leads to a pure integral control action, which discrete-time model sampled at $f_{s2}$, reads
\begin{equation}
\mathbf K(z) = \frac{k_j}{z-1},
\label{eq:K}
\end{equation}
where $k_j\in\mathbb R_+$ is the integral gain, computed by the proposed \textbf{L-DDC} procedure. Figure \ref{fig:K} shows the responses of the ideal control, as well as the reduced integral control obtained with $r=1$ (continuous and discrete), and compare it to the order $r=3$ one. Note that the control order remains a parameter that the designer can choose according to its implentation limitations. Here the simple integral choice has been considered as a good trade-off between complexity and performances.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./OL_gain.pdf}
    %\includegraphics[width=\columnwidth]{./figures/OL_phase}
    \caption{Gain of the frequency responses of the ideal controller $\mathbf K^\star$ evaluated at the available frequencies (blue dots), of the estimated controller $\mathbf{\tilde K}(s)$ of order $r=1$ (dotted magenta), $r=3$ (dashed green) and its discrete version $\mathbf K(z)$ (solid red).}
    \label{fig:K}
\end{figure}

\paragraph{Preliminary verification}

%Ici je vais mettre la BF estimée à partir des données et du controlleur 

The reduction of the controller model implies that the  closed-loop, denoted $\mathbf{T_{K}}$, obtained when inserting the reduced and sampled-time $\mathbf{K}$ controller, will not be equal to the desired reference model $\mathbf{M}$. Therefore, it is interesting to compute the frequency response of the expected closed-loop $\mathbf{T_{K}}$ on the basis of the available open-loop data $\{\imath\omega_i,\mathbf{\Phi}_i\}_{i=1}^N$ from the system as follows, $\forall i=1\dots N$
\begin{equation}
     \mathbf{T_{K}}(\imath \omega_i)=(I+\mathbf{\Phi}_i\mathbf{ K}(e^{\imath \omega_iT_{s2}}))^{-1}\mathbf{\Phi}_i\mathbf{ K}(e^{\imath \omega_iT_{s2}}).
    \label{cl_estimate}
\end{equation}

%The result is visible on Figure \ref{fig:clEstimated}, illustrating a promising performance. Note that for $r=3$, authors consider the gain not enough with respect to experimental benefits of a simple integral structure.
The result of the expected closed-loops for three different controllers is illustrated later on Figure \ref{fig:CL_freq}. Note that for $r=3$, authors considered that the gain was not important enough with respect to experimental benefits of such a simple integral structure, and is therefore not illustrated.

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{./figures/CLest_gain}
%    \caption{Estimated closed-loop performances using the computed $\mathbf{K}_1$ (without \textbf{PWM} block). Its stable projection fits the response of the estimated closed-loop, indicating that the resulting closed-loop is stable.}
%    \label{fig:clEstimated}
%\end{figure}

\paragraph{About stability}

% QQ remarque sur la stabilité (estimation basée données)

The choice of the reference model presented earlier ensures that the ideal controller stabilises the system internally. However, there is no stability guarantee regarding the use of a reduced-order controller. In \cite{KergusLCSS:2019}, the small-gain theorem is derived in a data-driven way: it is shown that limiting the controller modelling error during the reduction step ensures internal stability. This stability test is very conservative and another solution would be to use the projection-based technique of \cite{cooman2018model} or the one in \cite{PoussotHDR:2019} to conclude regarding the stability of the closed-loop. However, in the present case, as the considered actuator-sensor couple describes a positive system (\ie for any positive input, the output is positive), one can also exploit one result in \cite{BriatSIAM:2020}, which shows that such family of systems is stabilisable by an integral action only (authors skip the details here; future works out the scoope of this paper will consider this characteristics). 

%As for the choice of the reference model, this last option is used here. The projection the closed-loop data, built through \eqref{cl_estimate}, are interpolated to obtain a minimal realisation, which is then projected on $\Hinf$. The results, visible on \ref{fig:clEstimated}, indicates that the resulting closed-loop is stable.




==> sec_result.tex <==
\subsection{Considered configurations}

Based on the presented control design rationale and preliminary validation procedures presented in Section \ref{sec:method}, we are now ready to implement and validate the control setup on the real experimental test bench. The real-time acquisition and control functions, including the control law $\mathbf{K}(z)$, the \textbf{PWM} and \textbf{Average} blocks as schematized on Figure \ref{fig:closedLoopScheme}, are implemented within a LabView interface. For the considered flow system, three different controllers denoted $\mathbf{K_{f_j}}(z)$ with the same structure as in \eqref{eq:K}, sampled at $f_{s2}=100$Hz, corresponding to three different performance objectives $\mathbf{M_{f_j}}(s)$ as defined in \eqref{reference_model}, for $j=\{1,3,5\}$, are constructed. These may be read as,
\begin{itemize}
    \item $\mathbf{K_{f_1}}$, where $k_1 = 0.0462$ ($\mathbf{M_{f_1}}$ with $f_1=1$Hz),
    \item $\mathbf{K_{f_3}}$, where $k_3 = 0.1385$ ($\mathbf{M_{f_1}}$ with $f_3=3$Hz), and
    \item $\mathbf{K_{f_5}}$, where $k_5 = 0.2309$ ($\mathbf{M_{f_1}}$ with $f_5=5$Hz).
\end{itemize}
For the considered application, following Figure \ref{fig:closedLoopScheme} notations, $N=10$ and thus $f_{s1}=1000$Hz were chosen. The closed-loop performances are first validated with a sine sweep signal and second, with a more realistic reference trajectory.

\subsection{Closed-loop sine sweep reference signal}

We first apply a reference signal $\mathbf r(t_k)$ being a frequency sweep from $0.1$Hz to $30$Hz, of duration $1000$s and amplitude ranging from the minimal to the maximal possible values of the system. The mean values $\overline{\mathbf{y_{f_j}}}(t_k)$\footnote{Signal $\overline{\mathbf{y_{f_j}}}(t_k)$ refers to $\overline{\mathbf{y}}(t_k)$ on Figure \ref{fig:closedLoopScheme}, for $j$-th the configuration ($j=\{1,2,3\}$).} for all three configurations and time-domain responses are first reported on Figure \ref{fig:CL_time} and compared with the reference signal $\mathbf r(t_k)$. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./CL_time.pdf}
    \caption{Closed-loop time-domain response to a sine sweep in frequency. In black, the reference signal $\mathbf r(t_k)$ and in coloured shade, the different mean output values $\overline{\mathbf{y_{f_j}}}(t_k)$ (corresponding to $\overline{\mathbf{y}}(t_k)$ on Figure \ref{fig:closedLoopScheme}) for different $\mathbf{K_{f_j}}$ controllers (corresponding to $\mathbf{K}$ on Figure \ref{fig:closedLoopScheme}).}
    \label{fig:CL_time}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./CL_gain.pdf}\\
    \includegraphics[width=\columnwidth]{./CL_phase.pdf}
    \caption{Comparison of the gain (top) and phase (bottom) of the closed-loop frequency-domain responses of $\mathbf{T_{ry_{f_j}}}$ (from $\mathbf r$ to $\overline{\mathbf{\overline{y_{f_j}}}}$), obtained with the designed controllers $\mathbf{K_{f_j}}$, compared to the expected closed-loops $\mathbf{T_{K_{f_j}}}$.}
    \label{fig:CL_freq}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{./CL_tracking_u.pdf}
    \caption{Closed-loop response including $\mathbf{K_{f_1}}$, of the averaged output $\overline{\y}(t_k)$ (solid orange) to a variable reference trajectory $\mathbf r(t_k)$ (dashed black). Averaged control signal $\overline{\u}(t_k)$ (dotted blue).}
    \label{fig:CL_tracking}
\end{figure}

The averaged output flow velocity is found to well track the reference signal considered. In all three cases, the low frequencies are well tracked, which is already an important result for \textbf{PFA} systems and in view of fluid flow control. One can also observe that the tracking is more accurate in high frequencies with the more aggressive controller $\mathbf{K_{f_5}}$, synthesized to target a bandwidth of $f_5=5$Hz, validating the reference model approach of the data-driven procedure. To assess the tracking accuracy and that the designed procedure follows the specified reference model $\mathbf{M_{f_j}}$ given in the specifications, the frequency responses of the different $K_i$ controllers are computed. Figure \ref{fig:CL_freq} compares the experimental frequency-domain responses from $\mathbf r$ to $\overline{\mathbf{y_{f_j}}}$, denoted $\mathbf{T_{ry_{f_j}}}$, with $\mathbf{T_{K_{f_j}}}$, the expected closed-loop computed in \eqref{cl_estimate}.

For each controllers, the resulting closed-loop $\mathbf{T_{r\overline{y_{f_j}}}}$ provides a similar frequency response trends as the one expected and illustrated with $\mathbf{T_{K_{f_j}}}$. Some differences persist but can fairly be attributed to the nonlinear and non-symmetric nature of the pulsed  actuator. Indeed, as illustrated in Figure \ref{fig:OLinout} and  shown later in the section, when a reference amplitude close to zero is requested, some stick-like behaviour are observed, leading to a loss of accuracy. At this point, it is still notable that the obtained control law, designed solely through the lens of a pure data-driven approach, provides the required performances.

\subsection{Closed-loop using realistic reference signals}

Now the validation through a frequency behaviour analysis has been done, let us demonstrate the efficiency of the proposed control with a more realistic reference signal $\mathbf r(t_k)$. Figure \ref{fig:CL_tracking}  shows the tracking performance of the mean output $\overline{\y}(t_k)$ and control $\overline{\u}(t_k)$ signals using the first controller $\mathbf{K_{f_1}}$\footnote{On Figure \ref{fig:CL_tracking}, indices are removed and notations are the one of Figure \ref{fig:closedLoopScheme}.}.

Clearly, Figure \ref{fig:CL_tracking} exposes really satisfactory results in terms of tracking which is particularly relevant considering such low cost pulsed actuator. As previously pointed, one can remark that some chattering artefact and difficulties appear when tracking in low amplitude references. This observation can be correlated to the asymmetric actuator characteristic and to a stick-like behaviour in the valve opening. Even though not in the scope of this study, one way to limit this effect is to add high frequency noise in the control signal to avoid the problem, but at the price of an actuator fatigue (note that the approach is similar to solutions used in friction control). The averaged control signal $\overline{\u}(t_k)$ is also reported. % while the effective signal $\u(t_{k/N})$ is not given, being an on/off one hard to interpret. 
Interestingly, a simple integral controller action, obtained from a single open-loop data collection, using only on/off signals, allows tracking a complex reference signals with a good accuracy. 

==> sec_setup.tex <==

%Before detailing the construction of the feedback controller $\mathbf K(z)$, let us first present the setup, signals and \textbf{PWM} and \textbf{Mean} blocks. Such a description is essential to understand the results and is crucial to get successful experimental validation. %This last element playing a key role in the success of the approach. 

\subsection{Overall control setup}

%
%
A schematic view of the inner control loop is given in Figure \ref{fig:closedLoopScheme}. From a control engineer perspective, the flow control may be referred to as the outer-loop (out of this paper scope) while the pulsed fluidic actuator controller is referred to as the inner-loop. Following Figure \ref{fig:closedLoopScheme}, we are interested in the inner-loop only and more specifically in the control design, implementation and validation on a real \textbf{PFA}. With reference to Figure  \ref{fig:closedLoopScheme}, $\mathbf r(t_k)$ denotes the reference signal (typically the control signal provided by an outer controller) at time $t_k$,  $\overline\y(t_k)$ the measurement signal at time $t_k$ (typically the instantaneous velocity measured at the output of the \textbf{PFA}), $\mathbf e(t_k)=\mathbf r(t_k)-\overline\y(t_k)$ the error signal  at time $t_k$. Then $\overline{\u}(t_k)$ is the reference control signal computed at time $t_k$ by the sampled-time controller $\mathbf K(z)$ to be designed. Then,  $\u(t_{k/N})$ is the on/off control signal, at time $t_{k/N}$, modulated in pulse width by the Pulsed Width Modulation (\textbf{PWM}) block. The picture in Figure \ref{fig:closedLoopScheme} represents (left) the top view of the \textbf{PFA} and (right) the sensor probe, \textbf{PS}, sensing $\y(t_{k/N})$, here velocity, at time $t_{k/N}$, which is then down-sampled and averaged at time $t_{k}$, leading to $\overline{\y}(t_{k})$. As suggested on Figure \ref{fig:closedLoopScheme}, two sampling frequencies denoted as $f_{s2}$ and $f_{s1}=Nf_{s2}$ ($N\in\mathbb{N}$), referring to sampling times $t_{k/N}$ and $t_k$ respectively, are required to implement the controller. Details of this multi-sampling setup is given later in this section.

\subsection{Experimental setup}

%An experimental test bench has been set-up to demonstrate the proposed approach. 
The experimental test bench is composed of a \textbf{PFA} and a hot-wire probe (\textbf{PS}) as shown on the photo on Figure \ref{fig:closedLoopScheme}. The acquisition and generation of the command laws are carried out thanks to a real-time hardware system (National Instruments NI PXI-1042 mainframe).

The \textbf{PFA} used in the present study is a SX11F-BH micro-valve from SMC which can operate, according to the manufacturer, up to 1 kHz at a mean flow rate of 50 L/min. The asymmetric response times at opening and closing, again according to the manufacturer, are $0.55$ms and $0.4$ms respectively. For the present purpose, the valve is alimented with compressed air at constant pressure ($2.2$bar). A short tube of $D=5$mm diameter is used at the valve exit. The instantaneous velocity at $3D$ downstream the tube exit is surveyed thanks to a hot-wire probe (Dantec 55P11) connected to a 55M10 DISA constant temperature anemometer (CTA). Note that since the purpose of the present paper is to demonstrate the potential of the methodology introduced, no calibration of the hot-wire probe is effected. The voltage of the hot-wire probe is therefore directly considered as representative of the exit velocity and used as the output signal $\y(t_{k/N})$. From an application point of view, \textbf{PFA} equipped with outflow velocity sensors need to be developed (here an external hot-wire probe system is used).  This is currently being investigated in the Micro Opto Electro Mechanical Systems (MEMS) community. 

%Acquisition and communications hardware  allow for the interconnection with a LabView interface.

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{./figures/top}
%    \caption{Top view of the pulsed flow actuator (left) and hot %string measurement sensor (right).}
%    \label{fig:photoTop}
%\end{figure}
%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{./figures/side}
%    \caption{Side view of the pulsed flow actuator (left) and hot string sensor (right).}
%    \label{fig:photoSide}
%\end{figure}

%\noindent
%More specifically, the hardware part of the setup is composed of \emph{(i)} a \textbf{PFA}, black element of the left side of Figure \ref{fig:photoSide}, fed by constant level of compressed air (flexible red pipe), blowing at the red/grey pipe extremity, and  \emph{(ii)} the \textbf{HSS}, white and grey steel element with two pics on the right side of Figure \ref{fig:photoSide}, sensing the flow blown by the actuator (to be controlled). Both elements are sampled with a frequency $f_1=5,000$Hz. While the \textbf{HSS} measures the air pressure in continuous, the \textbf{PFA} can only operate open (on) or closed (off). 

\subsection{Pulsed width modulation and average blocks}%Schematic view of the control loop and detailed notations}

As the \textbf{PFA} works with only on/off control, a \textbf{PWM} function has naturally been implemented on the software side of the setup to transform the sampled-time signal $\overline\u(t_k)$ provided by the controller $\mathbf K(z)$ into $\u(t_{k/N})$, a stair signal with varying length (or Duty Cycle $D$). In addition, in order to take into account for noise measurement, since the probe sensor is not ideal, an average block is introduced and which operates on the measurement signal. The following presents the \textbf{PWM} and \textbf{Average} blocks in details.
\bigskip

\subsubsection{PWM block} 

 The \textbf{PWM} block uses a rectangular impulsion signal taking values between $\u_{\text{min}}$ and $\u_{\text{max}}$ and which length is modulated. This modulation results in variation of the mean of the signal $\overline\u(t_k)$ to convert. If one considers an impulsion with a high frequency $f_{s1}$ and a duty cycle $D\in[0,1]$, the averaged value $\u^{\text{avg}}(t_{k})$ of the resulting signal is given by
\begin{equation}
\begin{array}{rcl}
     \u^{\text{avg}}(t_{k}) &=& \dfrac{1}{T_{s2}} \displaystyle\int_0^{T_{s2}} \overline\u(t_k) dt_k \\
     &=& \dfrac{1}{T_{s2}} \bigg( \displaystyle\int_0^{DT_{s2}} \u_{\text{max}} dt_k + \displaystyle\int_{DT_{s1}}^{T_{s2}} \u_{\text{min}} dt_k \bigg) \\
     &=& D \u_{\text{max}} + (1-D)\u_{\text{min}}, %\\
     %&=& D \u_{\text{max}} \text{ (for $\u_{\text{min}}=0$)}.
\end{array}
\label{eq:pwm}
\end{equation}
where $T_{s1}=1/f_{s1}$ and $T_{s2}=1/f_{s2}$. Obviously, the \textbf{PWM} should be sampled at rate $N$ times higher than that of the signal $\u(t_k)$ to be modulated (with $N\in\mathbb N$). In practical applications, a simple way to generate the \textbf{PWM} is to use the intersection method which simply requires a saw-tooth carrier signal denoted $\u_c(t_k)$, with frequency $f_{s2}$ and amplitude from $\u_{\text{min}}=\min \overline\u(t_k)$ to $\u_{\text{max}}=\max \overline\u(t_k)$, that should be compared to the incoming signal $\overline\u(t_k)$. When $\u_c(t_k)>\overline\u(t_k)$, then $\u(t_{k/N})=\u_{\text{max}}$, and $\u(t_{k/N})=\u_{\text{min}}$ otherwise. Note that in the present case, the carrier signal has the same frequency as the control signal $\overline\u(t_k)$.
\smallskip

\subsubsection{Average block} 

The average block consists in averaging the measurement value $\y(t_{k/N})$ over $N$ past samples. The resulting output is a down-sampled signal $\overline\y(t_k)$, which represents the averaged output to be controlled and that should track $\mathbf r(t_k)$. The main purpose of such block is to partially filter out measurement noise, making the averaged value $\overline{y(t_k)}$ more representative of the output state than the instantaneous value $\y(t_{k/N})$.

\subsection{Signals characteristics and specifications}

Now the experimental setup and \textbf{PWM}/\textbf{Average} blocks have been presented, let us summarize the signals characteristics as follows:
\begin{itemize}
    \item $\mathbf r(t_k)$ (sampled at $f_{s2}$), is the reference signal to be tracked. This signal is continuous and is fed by the outer control. For the considered future application of turbulence control, its bandwidth is below $f_c=5$Hz\footnote{Note that this bandwidth may be considered as way too slow for fluid engineer. Still, this does not affect the method and higher bandwidth will be consiered in future works.} %\fk{...[FK] WE SHOULD DISCUSS THIS. FOR THE TURBULENCE COMMUNITY, IT MAY BE VERY VERY TOO LOW...on devrait peut-être dire que pour le présent travail, cela n'a pas de répercussion sur la méthode, et que l'on y travaille...}//}
    The knowledge of this signal characteristics is essential in the construction of the objective performance $\mathbf{M_{f_j}}(s)$ (see Section \ref{sec:method}).
    \item $\y(t_{k/N}) \in [\y_{\text{min}}~\y_{\text{max}}]$ (sampled at $f_{s1}$), is the measurement signal obtained by the \textbf{PS}. It allows measuring the air flow velocity at the exit of the actuation. Note that the distance of the probe from the \textbf{PFA} exit has an impact on the control law by adding a delay in the time response of the device. This is an additional reason justifying for the data-driven approach: the design can be reproduced easily for different distances or/and different probe sensors. 
    \item $\overline\y(t_k) \in [\y_{\text{min}}~\y_{\text{max}}]$ (sampled at $f_{s1}$), is the averaged and down-sampled value of $\y(t_{k/N})$ on blocks of duration $1/f_{s1}$ .
    \item $\overline \u(t_k)\in [0~\u_{\text{max}}]$ (sampled at $f_{s2}$), is the control signal provided by the \textbf{PFA} controller to be modulated by the \textbf{PWM} block. The sampling frequency of this signal determines the carrier and frequency of the  \textbf{PWM}.
    \item $\u(t_{k/N})\in\{0,\u_{\text{max}}\}$ (sampled at $f_{s1}$), is the effective modulated (pulsed) control signal sent to the \textbf{PFA}. 
\end{itemize}

 In our configuration, the controller $\mathbf K(z)$ and the \textbf{PWM} modules respectively run at frequency $f_{s2}=100$Hz and $f_{s1}=1000$Hz (thus $N=10$ is the \textbf{PWM} multiplicity factor). Now the setup and signals characteristics have been introduced, let us describe the main result, namely the workflow adopted to obtain the controller $\mathbf K(z)$  structure an gains.
